FreshGNN: Reducing Memory Access via Stable Historical Embeddings for Graph Neural Network Training

A key performance bottleneck when training graph neural network (GNN) models on large, real-world graphs is loading node features onto a GPU. Due to limited GPU memory, expensive data movement is necessary to facilitate the storage of these features on alternative devices with slower access (e.g. CPU memory). Moreover, the irregularity of graph structures contributes to poor data locality which further exacerbates the problem. Consequently, existing frameworks capable of efficiently training large GNN models usually incur a significant accuracy degradation because of the currently-available shortcuts involved. To address these limitations, we instead propose FreshGNN, a general-purpose GNN mini-batch training framework that leverages a historical cache for storing and reusing GNN node embeddings instead of re-computing them through fetching raw features at every iteration. Critical to its success, the corresponding cache policy is designed, using a combination of gradient-based and staleness criteria, to selectively screen those embeddings which are relatively stable and can be cached, from those that need to be re-computed to reduce estimation errors and subsequent downstream accuracy loss. When paired with complementary system enhancements to support this selective historical cache, FreshGNN is able to accelerate the training speed on large graph datasets such as ogbn-papers100M and MAG240M by 3.4x up to 20.5x and reduce the memory access by 59%, with less than 1% influence on test accuracy.

==> 2related.tex <==
\item \textbf{DSP}. We remark upfront that DSP is a framework explicitly designed for the multi-GPU setting, while \system can optimize either single or multi-GPU scenarios, with our original results mostly focusing on the former (with the exception of Figure \ref{fig:overall-multi-gpu}).  That being said, in our revised \Cref{sec:eval-perf}, we now reproduce DSP results using the same hardware setting as other evaluation results.  For fast multi-GPU training, DSP utilizes GPU resources for graph sampling, partitioning the graph into different GPUs to save space for caching. However, according to our evaluation, although the computational aspect of sampling is faster, sampling introduces communication overhead as the graph structure is not locally available. Moreover, its cache policy is solely based on node features, which leads to smaller IO saving relative to the historical embedding cache used by \system. As a result, while DSP can roughly achieve target accuracy, it can only reach up to 50\% of \system throughput in multi-GPU training.
\item \textbf{BGL}. Unfortunately, the main component of BGL, the graph partitioner, is not open sourced as of the time of this writing.\footnote{\url{github.com/leodestiny/BGL\_NSDI2023/tree/main/examples/pytorch/graphsage/experimental/partition\_codes\#readme}} Therefore, we can only analyze the metrics reported in their paper as opposed to 
directly reproducing in a head-to-head manner.
In this regard, for \texttt{ogbn-papers100M}, the reported BGL test accuracy converges to 47\% and 49\% with GraphSAGE and GAT models, respectively.  These results, which are based on the same standard OGB splits and GNN model architectures as ours, represent a more than 15\% gap relative to the target accuracy ($\sim$66\%), and are therefore not competitive with other approaches. In contrast, \system can efficiently converge to within 1\% of the target as shown in Table \ref{tab:overall}, making it more practically-relevant than BGL in terms of accuracy.  As for system performance, BGL and \system have different hardware settings, so head-to-head comparison is not feasible at this time.

==> algorithm/check.tex <==
\begin{algorithm}[ht]
\caption{Historical cache operations.}
\label{alg:check}
\begin{algorithmic}[1]
% \State {\bf Input}: History Table $\m{T}$, Embedding $h$, Gradient $grad$, Node set \m{V}

% \Function{LookUp}{$\m{T}$, $\m{V}_{in}$}
% % \State $ \m{V}_{history} \leftarrow  \{v, \forall v \in (\m{T} \cap \m{V}_{in} ) $ \} \label{line:lookup-prob}
% \State $ \m{V}_{history} \leftarrow \m{T} \cap \m{V}_{in}$ \label{line:lookup-prob}
% \State {\Return{$\m{V}_{history}$}}
% \EndFunction

\Function{CheckIn}{$\m{T}^l$, $\m{V}_{normal}^l$, $h^l$, $t$}
\For {$v \in \m{V}_{normal}^l$}
\If{$\m{T}^l.is\_full()$}
\State{$\m{T}^l.pop\_front()$} %\algorithmiccomment{First-In-First-Out}
\EndIf{}
\State{$\m{T}^l.push\_back(v, h_v^l)$}
\State{$t_{in}^l[v] \leftarrow t_{curr}$}
\EndFor
\EndFunction

\State {}

\Function{CheckOutStaleness}{$\m{T}^l, \m{V}_{cache}^l, t, staleness$}\label{line:staleness-eviction}
\State $ \m{T}^l \leftarrow \m{T}^l \setminus \{v\},
\forall v \in \m{V}_{cache}^l : t_{curr} - t^l_{in,v} > staleness$
\EndFunction

\State {}

% \Function{CheckOutGradient}{$\m{T}$, $\m{V}_{history}$, $grad$, $rate$} \label{line:gradient-eviction}
% \State $score \leftarrow one\_norm(grad) $
% \State $threshold_{grad} \leftarrow percentile(score, rate)  $ 
% \State $ \m{T}.delete(v), \forall v \in \m{V}_{history} : score_{v} \geq threshold_{grad} $
% \EndFunction

\Function{CheckOutGradient}{$\m{T}^l$, $\m{V}_{\m{G}_b}^l$, $rate$} \label{line:gradient-eviction}
\State $grad_v \leftarrow \|\nabla_v \ell\|, \forall v \in \m{V}_{\m{G}_b}^l$
\State $threshold \leftarrow percentile(grad, rate)  $ 
\State $\m{T}^l \leftarrow \m{T}^l \setminus \{v\}, \forall v \in \m{V}_{history} : grad_{v} \geq threshold$
\EndFunction

\State {}

\Function{CheckOut}{$\m{T}^l$, $\m{V}_{\m{G}_b}^l$, $t$, $rate$, $staleness$}
    \State \Call{CheckOutStaleness}{$\m{T}^l$, $\m{V}_{cache}$, $t$, $staleness$}
    \State \Call{CheckOutGradient}{$\m{T}^l$, $\m{V}_{\m{G}_b}^l$, $rate$}
\EndFunction

\end{algorithmic}
\end{algorithm}

==> algorithm/lookup.tex <==
% \begin{algorithm}[h]
% \caption{History table lookup.}
% \label{alg:lookup}
% \begin{algorithmic}[1]
% % \State {\bf Input}: History Table $\m{T}$, Embedding $h$, Gradient $grad$, Node set \m{V}
% \end{algorithmic}
% \end{algorithm}

==> other-eval.tex <==
\section{Other Evaluation Results}

\begin{figure}[h!]
\centerline{\includegraphics[width=0.48\textwidth]{fig/acc-curve.pdf}}
\caption{Convergence comparison w/ and w/o selective historical cache}
\label{fig:acc-curve}
\end{figure}



\begin{figure}
     \centering
     \begin{subfigure}[b]{0.23\textwidth}
        \centering
		\includegraphics
		[width=\textwidth]{fig/acc-stale.pdf}
		\caption{Staleness cache strategy\\\ }
		\label{fig:acc-stale}     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.23\textwidth}
        \centering
		\includegraphics
		[width=\textwidth]{fig/acc-stale+grad.pdf}
		\caption{Staleness and gradient cache strategy, staleness=200}
		\label{fig:acc-stale-grad}
     \end{subfigure}
\caption{Test accuracy for staleness and gradient cache strategy}
\label{fig:acc-breakdown}
\end{figure}

\begin{table}[ht]
\centering
\caption{Number of clusters and staleness for historical embeddings}
\footnotesize
\label{tab:eval-staleness-cluster}
\begin{tabular}{@{}lllllll@{}}
\toprule
\#Clusters                                                               & 250    & 500    & 1000   & 2000   & 4000    & 8000    \\ \midrule
Staleness                                                               & 104.14 & 208.30 & 416.30 & 830.92 & 1658.06 & 3309.79 \\
Data move (GB) & 31.65  & 17.30  & 7.50   & 3.93   & 1.37    & 0.80    \\ \bottomrule
\end{tabular}
\end{table}

\begin{figure}[h]
\centerline{\includegraphics[width=0.4\textwidth]{fig/breakdown.pdf}}
\caption{Performance improvement breakdown}
\label{fig:eval-breakdown}
\end{figure}

==> proof.tex <==


\section{Remarks on \system Convergence}
In this section, we analyze the convergence of the single-layer SGC model using a historical cache with a decoupled loss.

\subsection{Model and Notations}
Given a graph $\mathcal{G}=(\mathcal{V}, \mathcal{E})$ with $n$ nodes, the adjacency matrix is $A\in \R^{n\times n}$ and the available feature matrix is $X\in \R^{n\times d}$, where $d$ is the feature dimension. The normalized adjacency matrix for graph propagation is defined as $\hat A=(D+I)^{-\frac{1}{2}}(A+I)(D+I)^{-\frac{1}{2}} \in \R^{n \times n}$, $D_{u,u}=\sum_v A_{u,v}$.

The SGC model can be formulated as 
\begin{equation}
    Z=\hat{A}^k X W.
\end{equation}
Here the $Z$ and $W$ denote the embedding matrix and the weight matrix, respectively. For simplicity, we refer to $\hat{A}^k X$ as $\hat X$.

For the historical cache, we use a random selector to determine the staleness of the historical embedding we use for a node, where 0 staleness means not using historical embeddings. The series of matrices $S$ are diagonal binary matrices indicating whether or not to use a historical embedding and which one to use. $S_0$ selects the nodes that are calculated from neighbor aggregation, i.e. not using history, while $S_\tau,\tau=1,\cdots,s$ select the historical embeddings with corresponding staleness. So the historical model is:
\begin{align}
    % \tilde Z^{(0)}&=\hat{A}^k X W^{(0)} \\
    \tilde Z^{(0)}\!\!=\hat X W^{(0)}\text{; }
    % \tilde Z^{(t)}&=S_0\hat{A}^k X W^{(t)}
    \tilde Z^{(t)}\!\!=S_0^{(t)}\hat X W^{(t)}
    \!\!+\!\!\sum_{\tau=1}^s S_\tau^{(t)} \tilde Z^{(t-\tau)} \text{;}
    \sum_{\tau=0}^s S_\tau^{(t)} \!\!= I
    \label{analysis:historical-model}
\end{align}
Here $s$ is the maximum threshold for the staleness of historical embeddings. We assume $S$ are random and can be different at different iteration $t$. They are constructed as follows: $\xi_1, \xi_2, \cdots, \xi_n$ are independent and identically distributed with $\mathbb P(\xi_i=\tau)=p_\tau, \tau=0,1,\cdots,s, i=1,2,\cdots,n$, and $\sum_{\tau=0}^s p_\tau = 1$. The $i$-th element in the diagonal of $S_\tau$, $S_{\tau,ii}=\mathbb I_{\{\xi_i=\tau\}}$, where $\mathbb I$ is the indicator function. So $\mathbb E \left[S_{\tau,ii}\right]=\mathbb E \left[\mathbb I_{\{\xi_i=\tau\}}\right]=p_\tau$ and $\mathbb E\left[S_\tau\right]=p_\tau I$. It can be easily shown that $S_i S_j=S_i\cdot \mathbb I_{\{i=j\}}$

\subsection{Loss Functions}
% Given an embedding $Z_i$ and label $Y_i$ for node $i$, we define 
Suppose we have a metric function $\mathcal{L}$ with respect to the embedding $Z$ and label $Y$, we can define the loss function of $W$ as $\ell(W)=\mathcal{L}(Z,Y)=\sum_{i=1}^n \mathcal{L}(Z_i ,Y_i)$ and $\tilde \ell(W)=\mathcal{L}(\tilde Z,Y)=\sum_{i=1}^n \mathcal{L}(\tilde Z_i,Y_i)$. 

Note that here the $Z$ in the loss function $\ell$ is the embedding calculated without using history. In the historical model, we are using $\nabla\tilde\ell(W)$ for the update of parameter, and we want to show that it can still make $W$ converge in $\ell(W)$ thought it is not the real gradient of $\ell(W)$.

\begin{assumption}
\label{assum:lipschitz}
The loss function $\ell(W)$ is $L$-smooth w.r.t. $W$, i.e. $\|\nabla \ell(W^+)-\nabla \ell(W)\|_F \le L\|W^+-W\|_F$.
\end{assumption}

% \begin{assumption}
% \label{assum:decoupling}
% The loss function is decoupling for the input embeddings: $Loss(Z,Y)=\sum_{i=1}^n Loss(Z_i, Y_i)$
% \end{assumption}

\subsection{Proof of the Main Proposition}
\begin{prop}
Under Assumption \ref{assum:lipschitz}, for the historical model in \cref{analysis:historical-model}, if we use a fixed step size $\eta=\frac{1}{L}$, then the weight $W$ will converge to a stationary point of $\ell(W)$.
\end{prop}

\begin{proof}
At timestamp $t>1$,
\begin{align*}
    Z^{(t)}=\hat X W^{(t)} \text{; }
    \tilde Z^{(t)}=S_0^{(t)}\hat X W^{(t)}+\sum_{\tau=1}^s S_\tau^{(t)} \tilde Z^{(t-\tau)}.
\end{align*}

Since $S_i S_j=S_i\cdot \mathbb I_{\{i=j\}}$, we have $S_0^{(t)} Z^{(t)}=S_0^{(t)} \tilde Z^{(t)}$. This means
\begin{equation*} 
% & {\left[S_0^{(t)} \nabla_{Z^{(t)}} \mathcal{L}(Z^{(t)}, Y)\right]_{i,:} } = 
\nabla_{Z_i^{(t)}} \mathcal{L}(Z_i^{(t)}, Y_i) \cdot \mathbb I_{\left\{S_{0, i i}^{(t)}=1\right\}} 
=\nabla_{\tilde{Z}_i^{(t)}} \mathcal{L}(\tilde{Z}_i^{(t)}, Y_i) \cdot \mathbb{I}_{\left\{S_{0, i i}^{(t)}=1\right\}} 
% = {\left[S_0^{(t)} \nabla_{\tilde{Z}^{(t)}} \mathcal{L}(\tilde{Z}^{(t)}, Y)\right]_{i,:} }.
\end{equation*}

Therefore, 
% \begin{equation*}
$
    S_0^{(t)} \nabla_{Z^{(t)}} \mathcal{L}(Z^{(t)}, Y)=
    S_0^{(t)} \nabla_{\tilde{Z}^{(t)}} \mathcal{L}(\tilde{Z}^{(t)}, Y).$
% \end{equation*}

The gradient of $\ell(W^{(t)})$ is 
% \begin{equation*}
$
    \nabla\ell(W^{(t)})=\hat X^\top \nabla_{Z^{(t)}} \mathcal{L}(Z^{(t)}, Y),$


while the ``gradient'' we use for updating the parameter is
\begin{align*}
    \nabla \tilde \ell(W^{(t)})\!
    =\hat X^\top S_0^{(t)} \nabla_{\!\!\tilde{Z}^{(t)}}
    \mathcal{L}(\tilde{Z}^{(t)}, Y)\!
    =\hat X^\top S_0^{(t)} \nabla_{\!\!Z^{(t)}}
    \mathcal{L}(Z^{(t)}, Y). \label{analysis:grad}
\end{align*}

So the update rule for $W$ is
\begin{align*}
    W^{(t+1)} &\leftarrow 
    % W^{(t)}-\eta \hat X^\top S_0^{(t)} \nabla_{\tilde{Z}^{(t)}}
    % \mathcal{L}(\tilde{Z}^{(t)}, Y) \\
    W^{(t)}-\eta \hat X^\top S_0^{(t)} \nabla_{Z^{(t)}}
    \mathcal{L}(Z^{(t)}, Y).
\end{align*}

Since $\ell$ is Lipschitz smooth, it holds true that
\begin{align*}
\ell(W^{(t+1)})\!
% \leq&  \ell\left(W^{(t)}\right)+\left\langle\nabla \ell\left(W^{(t)}\right), W^{(t+1)}-W^{(t)}\right\rangle \\
% & +\frac{L}{2}\left\|W^{(t+1)}-W^{(t)}\right\|_F^2 \\
% &=\ell\left(W^{(t)}\right)-\eta\left\langle\nabla\ell\left(W^{(t)}\right), \nabla \tilde{\ell}\left(W^{(t)}\right)\right\rangle+\frac{L \eta^2}{2}\left\|\nabla \tilde{\ell}\left(W^{(t)}\right)\right\|_F^2 \\
\leq& \ell(W^{(t)})\!-\!\eta\!\left\langle\!\nabla \ell(W^{(t)}), \hat{X}^{\!\top}\!\!S_0^{(t)} \nabla_{\!\!Z^{(t)}} \!\mathcal{L}(Z^{(t)}\!, Y)\right\rangle \\
&+\frac{L \eta^2}{2}\left\|\hat{X}^{\top} S_0^{(t)} \nabla_{Z^{(t)}} \mathcal{L}(Z^{(t)}, Y)\right\|_F^2.
\end{align*}

Take expectation for $S_0^{(t)}$, we have
\begin{align*}
& \mathbb{E}\left[\ell(W^{(t+1)}) \mid W^{(t)}\right] \\
\le& \ell(W^{(t)})-\eta\left\langle\nabla \ell(W^{(t)}), \hat{X}^\top \mathbb E\left[S_0^{(t)}\right] \nabla_{Z^{(t)}} \mathcal{L}(Z^{(t)}, Y)\right\rangle \\
&+\frac{L \eta^2}{2}\left\|\hat{X}^{\top} \mathbb{E}\left[S_0^{(t)}\right] \nabla_{Z^{(t)}} \mathcal{L}(Z^{(t)}, Y)\right\|_F^2 \\
&+\frac{L \eta^2}{2} tr\left(\nabla_{Z^{(t)}} \mathcal{L}^\top\left(Var\left[S_0^{(t)}\right]\odot(\hat{X}\hat{X}^{\top})\right)\nabla_{Z^{(t)}} \mathcal{L}\right)\\
% \le& \ell(W^{(t)})-\eta p_0\left(1-\frac{L \eta p_0}{2}-\frac{L \eta (1-p_0)}{2}\right)\left\|\nabla \ell(W^{(t)})\right\|_F^2 \\
\le& \ell(W^{(t)})-\eta p_0\left(1-\frac{L \eta}{2}\right)\left\|\nabla \ell(W^{(t)})\right\|_F^2.
\end{align*}

Then by the law of total expectation, 
\begin{align*}
& \mathbb E\left[\ell(W^{(t+1)})\right]=\mathbb E\left[\mathbb E\left[\ell(W^{(t+1)}) \mid W^{(t)}\right]\right] \\
\le& \mathbb E\left[\ell(W^{(t)})\right]-\eta p_0\left(1-\frac{L \eta}{2}\right)\left\|\mathbb E\left[\nabla \ell(W^{(t)})\right]\right\|_F^2.
\end{align*}

So,
\begin{align*}
% &\left\|\mathbb E\left[\nabla \ell(W^{(t)})\right]\right\|_F^2 
%  \leq \frac{\mathbb E\left[\ell(W^{(t)})\right]-\mathbb E\left[\ell(W^{(t+1)})\right]}
% {\eta p_0\left(1-\frac{L \eta}{2}\right)};\\
% &\sum_{t=0}^T\left\|E\left[\nabla \ell(W^{(t)})\right]\right\|_F^2 
% \leq \frac{\ell(W^{(0)})-\ell(W^*)}{\eta p_0\left(1-\frac{L\eta}{2}\right)};\\
\min _{t=0, \cdots T}\left\|\mathbb E\left[\nabla \ell(W^{(t)})\right]\right\|_F^2 
% \leq& \frac{1}{T+1} \sum_{t=0}^T\left\|E\left[\nabla \ell\left(W^{(t)}\right)\right]\right\|_F^2 \\
\leq \frac{\ell(W^{(0)})-\ell(W^*)}{(T+1) \eta p_0\left(1-\frac{L\eta}{2}\right)}.
\end{align*}

Finally, as the iteration number satisfies $T\rightarrow\infty$, the expected gradient of the loss goes to $0$, and thus the convergence of the historical model to a stationary point is guaranteed.
\end{proof}

% Of course, this regime is admittedly quite limited, and not representative of more nuanced behavior involving the coupling of node embeddings of varying degrees of staleness across different layers. Although some prior analysis of gradient descent with stale features and gradients does exist \cite{pipegcn, dorylus, vrgcn}, the setting is decidedly much simpler and does not directly apply to our complex modeling framework; however, we can consider potential adaptations in future work.  As a point of reference though, most GNN models with adjustments for scalability (e.g., various sampling methods) do not actually come with any rigorous convergence guarantees.  

==> revision.tex <==
\newcommand{\rereq}[1]{\noindent \textcolor{black}{ \bf #1: }\xspace}
% \newcommand{\reans}[1]{\noindent \textcolor{revisioncolor}{ Response\##1: }\xspace}
\newcommand{\reans}[1]{\vspace{-.05in}\noindent { Response: }\xspace}
\newcommand{\boxrv}[1]{\textcolor{black}{#1}}
\newcommand{\comments}[1]{\textcolor{red}{#1}}
\newcommand{\other}{\subsection*{\textcolor{revisioncolor}{Response to other comments: }}\xspace}


\newcommand{\problemvspace}{\vspace{.1in}}

\twocolumn[
\begin{@twocolumnfalse}
% \vspace{0.1in}
{\centering \part*{\bf \Huge Response to Reviewer Comments}}
Dear anonymous reviewers,

\hspace{2mm}We sincerely appreciate the valuable comments
and suggestions that have helped us greatly improve the paper. 
The modifications we have made to the revised paper are highlighted 
in \revision{blue color}, with (temporary) blue labels in the margin to reference which rebuttal comment is being addressed by the new content. For example, \revision{4-1} represents our response to Reviewer\#4 Comment1.
We also address the review summary and each reviewer comment in detail below.

\vspace{0.1in}
\hrule
\hrule
\vspace{0.1in}
\end{@twocolumnfalse}
]

% \problemvspace{}
\section*{ \underline{[Response to meta review]}}

\definecolor{shadecolor}{rgb}{0.9,0.9,0.9}

\begin{shaded}%
\rereq{M1: The motivation of this work}
\end{shaded}

\reans
% \david{I don't think we should use blue again for the word ``Response" since it kind of a different use case than what we describe the blue color for above.} 
\boxrv{
We made the following modifications to make the motivation behind our designed system clearer:
}
% \begin{enumerate}
\begin{enumerate}[itemsep=0pt, parsep=0pt, labelsep=5pt,leftmargin=*, topsep=0pt,partopsep=0pt]
    \item \para{Sampling overhead}. We revised statements related to the graph sampling experiment in \Cref{sec:eval} to eliminate potential misunderstandings. We now clearly state that the time allocated to sampling has been optimized to a minimal level, which is overlapped by training time. So the bottleneck still lies in data loading, necessitating the implementation of \system's historical cache mechanism to reduce and optimize data loading.
    \item \para{Initial instability}. 
    % \david{Is this part really a motivation of our work?} 
    {\system is motivated by embedding stability, however, the embeddings may not be stable at the beginning of training.
    To address this issue,} 
    we introduced and conducted new experiments involving the use of a stabilization period in \Cref{sec:cache} and \Cref{sec:eval} respectively. After this period, the majority of embeddings remain stable, and \system employs a cache strategy for identifying these stable embeddings, accumulating historical embeddings, and reusing them to minimize data loading.
% It demonstrates how \system addresses the instability of embeddings during the initial training phase. After overcoming the initial training instability, a majority of embeddings become stable. Therefore 
    \item \para{Design of data loader}. We added more discussion on the motivation of the data loader design in \Cref{sec:data-loader}. 
    {We mention here that prior work } 
    % \david{This is not worded clearly; it could be interpreted as our previous design in the original submission, or previous design in the literature prior to the latter.  I believe the second case is our intended meaning, but this might not be clear to readers.} 
    initiates data loading from CPU and performs it ahead of each iteration. 
    % \david{Of what?  Advance of training?}\cg{changed} 
    However, this design cannot work well with a historical cache, as it is updated in real-time and by GPUs. This motivates \system to design one-sided communication to initialize communication from GPU, and design scheduled communication to efficiently perform real-time data loading. 
\end{enumerate}

\begin{shaded}%
\rereq{M2: Enhance the experimental studies and compare with two missing related work}
\end{shaded}

\reans
\boxrv{
We mainly made the following updates to improve the evaluation:
}
\begin{enumerate}[itemsep=0pt, parsep=0pt, labelsep=5pt,leftmargin=*, topsep=0pt,partopsep=0pt]
    \item Comparison with missing related work, namely, the DSP and BGL frameworks.
    % \begin{enumerate}
    \begin{enumerate}[itemsep=0pt, parsep=0pt, labelsep=5pt,leftmargin=*, topsep=0pt,partopsep=0pt]
        % \item \textbf{DSP}. We remark upfront that DSP is a framework explicitly designed for the multi-GPU setting, while \system can optimize either single or multi-GPU scenarios, with our original results mostly focusing on the former (with the exception of Figure \ref{fig:overall-multi-gpu}).  That being said, in our revised \Cref{sec:eval-perf}, we now reproduce DSP results using the same hardware setting as other evaluation results.  For fast multi-GPU training, DSP utilizes GPU resources for graph sampling, partitioning the graph into different GPUs to save space for caching. However, according to our evaluation, although the computational aspect of sampling is faster, sampling introduces communication overhead as the graph structure is not locally available. Moreover, its cache policy is solely based on node features, which leads to smaller IO saving relative to the historical embedding cache used by \system. As a result, while DSP can roughly achieve the target accuracy, it can only reach up to 50\% of \system throughput in multi-GPU training.\david{What about accuracy, is it similar to ours?}\revision{Yes, similar accuracy.}\david{Then should we mention this?}\revision{added}
        % \item \textbf{BGL}. Unfortunately, the main component of BGL, the graph partitioner, is not open sourced as of the time of this writing.\footnote{\url{github.com/leodestiny/BGL\_NSDI2023/tree/main/examples/pytorch/graphsage/experimental/partition\_codes\#readme}} Therefore, we can only analyze the metrics reported in their paper as opposed to directly reproducing in a head-to-head manner. In this regard, for \texttt{ogbn-papers100M}, the reported BGL test accuracy converges to 47\% and 49\% with GraphSAGE and GAT models.  This represents a more than 15\% gap relative to the target accuracy ($\sim$66\%), which is not competitive with other approaches. In contrast, on the same model and dataset,
        % \system can efficiently converge to within 1\% of the target as shown in Figure \ref{tab:overall}, making it more practically-relevant than BGL in terms of accuracy.
        %         \item \textbf{DSP}. We remark upfront that DSP is a framework explicitly designed for the multi-GPU setting, while \system can optimize either single or multi-GPU scenarios, with our original results mostly focusing on the former (with the exception of Figure \ref{fig:overall-multi-gpu}).  That being said, in our revised \Cref{sec:eval-perf}, we now reproduce DSP results using the same hardware setting as other evaluation results.  For fast multi-GPU training, DSP utilizes GPU resources for graph sampling, partitioning the graph into different GPUs to save space for caching. However, according to our evaluation, although the computational aspect of sampling is faster, sampling introduces communication overhead as the graph structure is not locally available. Moreover, its cache policy is solely based on node features, which leads to smaller IO saving relative to the historical embedding cache used by \system. As a result, while DSP can achieve target accuracy, it can only reach up to 50\% of \system throughput in multi-GPU training.
        % \item \textbf{BGL}. Unfortunately, the main component of BGL, the graph partitioner, is not open sourced as of the time of this writing.\footnote{\url{github.com/leodestiny/BGL\_NSDI2023/tree/main/examples/pytorch/graphsage/experimental/partition\_codes\#readme}} Therefore, we can only analyze the metrics reported in their paper as opposed to explicitly reproducing results. In this regard, for \texttt{ogbn-papers100M}, the reported BGL test accuracy converges to 47\% and 49\% with GraphSAGE and GAT models, respectively.  These results, which are based on the same standard OGB splits and model architectures as ours, represents a more than 15\% gap relative to the target accuracy ($\sim$66\%), and is therefore not competitive with other approaches. In contrast, \system can efficiently converge to within 1\% of the target as shown in Table \ref{tab:overall}, making it more practically-relevant than BGL in terms of accuracy.
        \input{2related}
    \end{enumerate}
    \item \textbf{More ablation study}. In \Cref{subsec:ablation}, we carry out further ablations to examine  the initialization overhead, how the number of layers and graph topology influence \system performance, and how \system avoids unstable embeddings at the beginning of training. These ablation studies serve to better evaluate how \system behaves with different model architectures and further showcase the practicality of \system.
\end{enumerate}

\begin{shaded}%
\rereq{M3: Additional analysis and discussion}. 
\end{shaded}

\reans{1} 
\boxrv{
We added  the following analysis and discussion to make the paper more sound.
}
\begin{enumerate}[itemsep=0pt, parsep=0pt, labelsep=5pt,leftmargin=*, topsep=0pt,partopsep=0pt]
\item \para{Discussion on other cache policies}. We include additional discussion of other cache policies in \Cref{sec:related}, including policies based on node features and historical embeddings;
\item \para{\system sensitivity to model and dataset}. We discussed and evaluated how \system performs with different model structure (number of layers) in \Cref{fig:eval-revision}(b) and graph dataset characteristics (node degrees and diameters) in \Cref{fig:eval-diverse-graph}.
% \david{Should mention where to find this.}\revision{added}
\end{enumerate}


\section*{ \underline{[Response to Reviewer \#4]}}


\begin{shaded}%
\rereq{4-1: Overhead of sampling process.}
Some modules within the system appear to require significant amounts of time, causing other modules to wait, e.g., sampling process consumes hundreds of seconds (\Cref{fig:eval-generator}) while training time is shorter (\Cref{fig:overall-single-gpu}).
\end{shaded}

\reans{1} 
\boxrv{
We apologize for any misunderstanding caused by our previous wording and illustrations for \Cref{fig:eval-generator}.
% \david{The reviewer also mentioned Figure 10, but that is not referenced in the response}\revision{added}. 
In fact, the \system sampling time is relatively small compared to the training time and can be overlapped by it. 
\Cref{fig:eval-generator} shows that although sampling takes hundreds of seconds with single CPU thread, increasing the number of CPU threads (to 32 threads) results in a significant reduction in sampling time to 11 seconds, which can be overlapped by the training time ($\sim$30 seconds as shown in \Cref{fig:overall-single-gpu}). We have updated \Cref{fig:eval-generator} and the related description to clarify this point.
% Sampling process consumes minor time and is overlapped by training time. \Cref{fig:eval-breakdown} shows that while sampling process takes hundreds of seconds with a single CPU thread, it can be accelerated by utlizing multiple CPU threads. With 32 CPU threads, the execution time of sampling is 8 seconds and can be overlapped by training time. We changed \Cref{fig:eval-breakdown} to highlight the final performance of sampling.
}

\begin{shaded}%
\rereq{4-2: Initial instability of embeddings.}
In Figure 3, it is evident that the cache and staleness policy employed in GNN training is not initially suitable. It is suggested that a dynamic scheduling approach may yield better results, which may need further evaluations.
\end{shaded}

\reans{1} 
\boxrv{
% \Cref{fig:cos-simlarity-emb} describes the similarity between node embeddings at different iterations. It demonstrates that some embeddings are unstable, leading to bad accuracy. As \system selectively caches part of the embeddings, it can avoid reusing such unstable embeddings. We added an ablation study to show \system's start stage. 
This is a helpful point to consider. In fact, this problem can be addressed with a simple strategy: only enabling the historical cache after training for a period of time, rather than enabling it from the very beginning. In this way, we can cache and reuse historical embeddings only after the unstable embedding phase. We refer to the period without enabling the historical cache as the \textit{stabilization period}. In new evaluations from in \Cref{tab:eval-cold-start} of the revision, we have now investigated the impact of the stabilization period on accuracy. These experiments show that on GraphSAGE, for \texttt{ogbn-papers100M}, where FreshGNN's accuracy is already close to the target accuracy (-0.15\%), the stabilization period has a minimal effect on accuracy. However, for \texttt{MAG240M}, introducing the stabilization period reduced the \system accuracy gap from -0.51\% to -0.12\%, demonstrating its effectiveness.  (We also note that the duration of the stabilization period is tiny relative to the overall number of training iterations, hence it has negligible impact on system performance.) As such, we have included an introduction to the stabilization period in \Cref{sec:cache}.  Thanks for the suggestion, which helps to improve our framework.
}

\begin{shaded}%
\rereq{4-3: Pre-processing overhead.}
The experiments do not include the pre-processing time required for certain tasks, such as calculating the memory access saved as described in Section 4.2.1.
\end{shaded}

\reans
\boxrv{
% We add an experiment in \Cref{sec:eval} to show that the pre-processing overhead is negligible compared with overall training time. The computation complexity of pre-processing overhead is $O(E)$, which $E$ is the number of edges in the graph data. As \system utilizes GPU to perform pre-processing, its throughput can reach up to xx edges per second, which takes only xx seconds for papers100M.
% \david{The response below needs revision and could be interpreted negatively by the reviewer.  Is the argument we are trying to make that the original submission already answered the reviewer's question?  The way it is currently worded, it is unclear whether new content has been added or that the original submission adequately handled this topc.  Also, it is not advisable to repeatedly claim that the overhead is acceptable.  Better to just provide the numbers the reviewer requests and then state once the significance.}\revision{rewritten}
% In \Cref{subsec:ablation}, we discussed the preprocessing overhead of \system and demonstrated that the overhead is acceptable. Firstly, in \Cref{fig:eval-revision}(b), we compared the pre-processing overhead with other necessary steps during training, such as loading node features from the disk (Disk2DRAM) and the training time for each epoch (Epoch time). We found that the pre-processing overhead is smaller compared to these steps. Additionally, for the same dataset, the pre-processing results can be reused multiple times. Therefore, the pre-processing overhead of \system is considered acceptable.
In \Cref{subsec:ablation}, we added an experiment to evaluate \system's pre-processing overhead. 
\Cref{fig:eval-revision}(b) illustrates various steps on the \texttt{ogbn-papers100M}, including loading node features from disk to DRAM before training (Disk2DRAM), the time taken for one epoch of training (Epoch time), and the pre-processing overhead of \system. It can be observed that compared to Disk2DRAM ($\sim$40s) and the periodically recurring training time ($\sim$30s per epoch), the pre-processing overhead ($\sim$9s) is not a significant factor. Additionally, the pre-processing results can be reused for the same dataset and training configuration.
}

\begin{shaded}%
\rereq{4-4: Differentiate the usage of models.}
The manuscript mentions the usage of GCN, GraphSAGE, and GAT models, but it does not clearly differentiate them in the experimental section.
\end{shaded}

\reans
\boxrv{
The evaluation mainly has two parts, including accuracy and performance tests. For accuracy, we test different models to evaluate \system's influence on model accuracy. For performance, as the bottleneck is data movement instead of computation, all evaluations are carried on GraphSAGE, and similar performance is observed on other models. Clarification has been added to \Cref{sec:eval}.
}

\begin{shaded}%
\rereq{4-5: Employed sampling method.}
Under Algorithm 1, it is mentioned to generate a subgraph based on a user-defined sampling method. However, the specific details of the sampling method employed in this paper are not provided.
\end{shaded}

\reans
\boxrv{
% The sampling method used in this paper is neighbor sampling~\cite{graphsage}, 
The base sampling method we adopt for mini-batch training is commonly-used neighbor sampling~\cite{graphsage}  following the setting of the OGB leaderboard~\cite{ogb} to set the neighbor sampling fan-out as 20, 15, and 10.  We have added clarification in \Cref{sec:overview} and \Cref{sec:eval}.
}

\begin{shaded}%
\rereq{4-6: Overall presentation quality.}
The overall presentation quality of the paper can be enhanced through proofreading.
\end{shaded}

\reans
\boxrv{
We have proofread the paper to enhance the presentation quality, including but not limited to the issues pointed out here.
}


\section*{ \underline{[Response to Reviewer \#5]}}


\begin{shaded}%
\rereq{5-1: Comparison to most recent work}
\end{shaded}

\reans
\boxrv{
We carried out comparison to the latest baselines, including DSP~\cite{dsp} and BGL~\cite{bgl}.
% \david{This response is inferior to the longer, more descriptive version presented to the meta-review.  Much better to either reference the original meta-review, or else copy and paste that version here (at least for ML conferences, it is not uncommon to reuse rebuttal materials in this way, noting that the reviewer may only read the rebuttal portion that relates to their review.).} \revision{I used the one from meta review}
% We carried out the comparison with DSP~\cite{dsp} and BGL~\cite{bgl} in \Cref{sec:eval}. Compared with DSP, \system can achieve 1.91$\times$ speedup on average; For BGL, as the core component is not publicly available, we analyze the metrics reported in the paper and find it will lead to over 15\% accuracy drop on \texttt{ogb-papers100M}, while \system can control all accuracy gap within 1\%.
}
    \begin{enumerate}[itemsep=0pt, parsep=0pt, labelsep=5pt,leftmargin=*, topsep=0pt,partopsep=0pt]
        % \item \textbf{DSP}. We remark upfront that DSP is a framework explicitly designed for the multi-GPU setting, while \system can optimize either single or multi-GPU scenarios, with our original results mostly focusing on the former (with the exception of Figure \ref{fig:overall-multi-gpu}).  That being said, in our revised \Cref{sec:eval-perf}, we now reproduce DSP results using the same hardware setting as other evaluation results.  For fast multi-GPU training, DSP utilizes GPU resources for graph sampling, partitioning the graph into different GPUs to save space for caching. However, according to our evaluation, although the computational aspect of sampling is faster, sampling introduces communication overhead as the graph structure is not locally available. Moreover, its cache policy is solely based on node features, which leads to smaller IO saving relative to the historical embedding cache used by \system. As a result, while DSP can achieve target accuracy, it can only reach up to 50\% of \system throughput in multi-GPU training.
        % \item \textbf{BGL}. Unfortunately, the main component of BGL, the graph partitioner, is not open sourced as of the time of this writing.\footnote{\url{github.com/leodestiny/BGL\_NSDI2023/tree/main/examples/pytorch/graphsage/experimental/partition\_codes\#readme}} Therefore, we can only analyze the metrics reported in their paper \david{Do they have any system performance metrics we could compare with?} as opposed to explicitly reproducing results. In this regard, for \texttt{ogbn-papers100M}, the reported BGL test accuracy converges to 47\% and 49\% with GraphSAGE and GAT models, respectively.  These results, which are based on the same standard OGB splits and model architectures as ours, represents a more than 15\% gap relative to the target accuracy ($\sim$66\%), and is therefore not competitive with other approaches. In contrast, \system can efficiently converge to within 1\% of the target as shown in Table \ref{tab:overall}, making it more practically-relevant than BGL in terms of accuracy.
        \input{2related}
    \end{enumerate}

\begin{shaded}%
\rereq{5-2: Graph topology and performance/accuracy tradeoff}
% Lacking analysis on how the topology of the graph will affect the performance/accuracy trade-off.
More datasets of various characteristics, e.g., different topologies, diameters, should be provided to understand the performance/accuracy tradeoff.
\end{shaded}

\reans
\boxrv{We agree that it is valuable to include a comprehensive set of benchmarks for comparison; however, for present purposes we note that there are limited options when it comes to large-scale public graph datasets with labels provided (i.e., such that accuracy can be evaluated).  In this regard, we have made a conscious effort to include the standard datasets commonly used in prior GNN scalability work, e.g., see \cite{dsp, p3, gnnlab, bgl} which collectively adopt benchmarks that are a subset of ours.  This overlap is important as it facilitates meaningful comparisons with published baseline models where possible. 



We understand the concern about the number of datasets and their impact on evaluating the impact of cache on the accuracy in \system. However, it is important to note that there is indeed a scarcity of large-scale public graph benchmarks {with labels provided (so that the accuracy can be evaluated)}, and we have made a conscious effort to include the standard datasets that are commonly used in prior work~\cite{dsp, p3, gnnlab, bgl}. These datasets are not only relevant but also allow for a meaningful comparison with published baseline models, which utilize a subset of the datasets we have employed.

Additionally, we have gone one step further by using two versions of the largest dataset available, \texttt{MAG240M}. This dataset is utilized in both a homogenized and a heterogeneous graph format within our paper.
% , \revision{which has more types of nodes and edges connected in different ways} \cred{(jht: a little bit ambiguous?)}. 
This dual approach allows us to explore and understand the impact of caching on accuracy within more diverse graph structures, {as the homogenized graph only contains paper nodes and citation links, while the heterogeneous one contains additional node types (e.g. authors and institutes) and relations/edges.}. Importantly, in both cases, the accuracy gap between \system and the target is negligible. Hence the use of \texttt{MAG240M} in these two formats adds a unique dimension to our study, helping to assess the robustness and flexibility of our caching mechanism across a broader scenario/topology.

% \david{This reviewer mentioned that we only used a limited number of datasets (only 4), but this is not actually even true. 
%  We actually tested accuracy on 5 when we include two versions of Mag, and we tested system performance on 6, including Twitter and Friendster.  I think it could be worth clarifying this point, and mentioning that there are very limited options for public large-scale graph datasets.  This would then help further motivate why we adopt synthetic experiments.}

% We address the issue of dataset divergence \david{Did you mean dataset diversity?} in terms of both performance and accuracy.

Beyond this, for more diverse testing across large-scale graph topologies, we are unaware of suitable additional benchmarks.  That being said, we can still at least synthesise graphs to evaluate the system performance of \system over different graph structures. Therefore, we conducted a comparison in \Cref{fig:eval-diverse-graph} by generating graphs with different topological characteristics to assess whether the historical cache employed by FreshGNN can still optimize data loading. Using the \texttt{ogb-papers100M} as the base graph, we modified the node degrees by adding or removing edges and changed the graph diameter by restricting the range of node connections (note that with these structural changes, accuracy is no longer a meaningful metric for evaluation). Upon testing with these graphs, our results indicate that while various graph topologies may significantly affect IO saving due to caching, FreshGNN's historical cache consistently outperforms feature caches.
% \david{What about graph diameter?}\cg{here it means the frequency of the nodes are determined by the node degree, which is used to decribe the feature cache policy. I will just remove "based on node degree" to avoid misunderstanding}
In scenarios where the graph exhibits diverse node degrees, the historical cache leads to an average IO saving of 1.56$\times$. Similarly, in scenarios where the graph has varying diameters, the historical cache results in an average IO saving of 1.43$\times$.

% We added the evaluation on graphs with different characteristics, including roadmap with high diameter.
}

\section*{ \underline{[Response to Reviewer \#6]}}


\begin{shaded}%
\rereq{6-1: Discussion on the caching policy of existing systems}
\end{shaded}

\reans
\boxrv{
We have added discussion on existing GNN caching policies  in \Cref{sec:related}. The discussion includes cache policies based on node features and historical embeddings. For node features, the focus of previous work is to accurately estimate the visiting frequency of the node features and cache the ones with high frequency. Methods include using node degrees, PageRank, and profiling~\cite{gnnlab,pagerank,pagraph,agnn,gnntier}. Turning to historical embedding usage, prior work either caches all intermediate nodes~\cite{vrgcn,gas} or the boundary nodes (in multi-GPU training)~\cite{sancus}. These un-selective methods can result in out-of-memory or low accuracy as we have shown.
Different cache policies are also evaluated for accuracy and IO saving  respectively in \Cref{sec:eval-acc} and \Cref{subsec:ablation}.
}

\begin{shaded}%
\rereq{6-2: The impact of number of layers on \system}
\end{shaded}

\reans{1} 
\boxrv{
% We added experiment on how number of layers influence performance of \system. Generally speaking, the performance of \system can be improved with more number of layer as more visit to nodes will be pruned by historical cache.
In practice, most large-scale GNN models have depth of 3 or smaller.  Nonetheless, we have conducted additional experiments to evaluate the capability of \system in handling GNN models with increasing depth. In \Cref{fig:eval-revision}(a), we present a comparison of \system's IO saving and feature cache for GNN models with a varying number of layers. These  results indicate that as the number of layers increases, and the number of accessed nodes rises, both types of cache lead to reduced IO saving. However, \system consistently maintains higher IO saving (1.50$\times$) compared to the feature cache based on node degree.
% \david{What alternative method?  Nothing has been specified here.}\revision{added}
}

\begin{shaded}
\rereq{6-3: The connection from \Cref{sec:subgraph-generator} to \Cref{sec:data-loader}}
\end{shaded}

% \david{The response below does not address the reviewers point.  He is making a suggestion for improving the paper, not requesting an explanation for the rebuttal.  Better to just say we have modified the text to clarify, or else argue for why clarification in the paper is not necessary.}\revision{fixed}

\reans
\boxrv{
We added more discussion to explain the motivation and necessity of data loader design in \Cref{sec:data-loader}. 
To make the flow more fluent, we emphasized the challenge brought by historical cache that it is the GPU instead of the CPU that prunes the subgraph and holds the ID of the node features needed for training.
% As shown in \Cref{fig:system-overview}, to support historical cache, \system needs to generate pruned subgraph and load the node features still used by it. These two steps are introduced in \Cref{sec:subgraph-generator} and \Cref{sec:data-loader} respectively. \Cref{sec:data-loader} introduces how \system initializes the data loading from GPU, which is essential for historical cache as the needed node IDs are only available on GPU. The performance and  necessity of the subgraph generator and data loader are evaluated in \Cref{subsec:ablation}.
}
